HyperKon: A Self-Supervised Contrastive Network for Hyperspectral Image Analysis

The exceptional spectral resolution of hyperspectral imagery enables material insights that are not possible with RGB or multispectral images. Yet, the full potential of this data is often underutilized by deep learning techniques due to the scarcity of hyperspectral-native CNN backbones. To bridge this gap, we introduce HyperKon, a self-supervised contrastive learning network designed and trained on hyperspectral data from the EnMAP Hyperspectral Satellite\cite{kaufmann2012environmental}. HyperKon uniquely leverages the high spectral continuity, range, and resolution of hyperspectral data through a spectral attention mechanism and specialized convolutional layers. We also perform a thorough ablation study on different kinds of layers, showing their performance in understanding hyperspectral layers. It achieves an outstanding 98% Top-1 retrieval accuracy and outperforms traditional RGB-trained backbones in hyperspectral pan-sharpening tasks. Additionally, in hyperspectral image classification, HyperKon surpasses state-of-the-art methods, indicating a paradigm shift in hyperspectral image analysis and underscoring the importance of hyperspectral-native backbones.

==> egbib.tex <==
@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})


@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})


@article{simonyan2014very,
  title={Very deep convolutional networks for large-scale image recognition},
  author={Simonyan, Karen and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1409.1556},
  year={2014}
}

@article{he2019hyperpnn,
  title={HyperPNN: Hyperspectral pansharpening via spectrally predictive convolutional neural networks},
  author={He, Lin and Zhu, Jiawei and Li, Jun and Plaza, Antonio and Chanussot, Jocelyn and Li, Bo},
  journal={IEEE Journal of Selected Topics in Applied Earth Observations and Remote Sensing},
  volume={12},
  number={8},
  pages={3092--3100},
  year={2019},
  publisher={IEEE}
}

@article{xie2020hpgan,
  title={HPGAN: Hyperspectral pansharpening using 3-D generative adversarial networks},
  author={Xie, Weiying and Cui, Yuhang and Li, Yunsong and Lei, Jie and Du, Qian and Li, Jiaojiao},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={59},
  number={1},
  pages={463--477},
  year={2020},
  publisher={IEEE}
}

@article{chen2016deep,
  title={Deep feature extraction and classification of hyperspectral images based on convolutional neural networks},
  author={Chen, Yushi and Jiang, Hanlu and Li, Chunyang and Jia, Xiuping and Ghamisi, Pedram},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={54},
  number={10},
  pages={6232--6251},
  year={2016},
  publisher={IEEE}
}

@inproceedings{bandara2022hypertransformer,
  title={HyperTransformer: A textural and spectral feature fusion transformer for pansharpening},
  author={Bandara, Wele Gedara Chaminda and Patel, Vishal M},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={1767--1777},
  year={2022}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@inproceedings{huang2017densely,
  title={Densely connected convolutional networks},
  author={Huang, Gao and Liu, Zhuang and Van Der Maaten, Laurens and Weinberger, Kilian Q},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={4700--4708},
  year={2017}
}
@inproceedings{sidorov2019deep,
  title={Deep hyperspectral prior: Single-image denoising, inpainting, super-resolution},
  author={Sidorov, Oleksii and Yngve Hardeberg, Jon},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision Workshops},
  pages={0--0},
  year={2019}
}

@article{zheng2019separable,
  title={Separable-spectral convolution and inception network for hyperspectral image super-resolution},
  author={Zheng, Ke and Gao, Lianru and Ran, Qiong and Cui, Ximin and Zhang, Bing and Liao, Wenzhi and Jia, Sen},
  journal={International Journal of Machine Learning and Cybernetics},
  volume={10},
  pages={2593--2607},
  year={2019},
  publisher={Springer}
}

@article{loncan2015hyperspectral,
  title={Hyperspectral pansharpening: A review},
  author={Loncan, Laetitia and De Almeida, Luis B and Bioucas-Dias, Jos{\'e} M and Briottet, Xavier and Chanussot, Jocelyn and Dobigeon, Nicolas and Fabre, Sophie and Liao, Wenzhi and Licciardi, Giorgio A and Simoes, Miguel and others},
  journal={IEEE Geoscience and remote sensing magazine},
  volume={3},
  number={3},
  pages={27--46},
  year={2015},
  publisher={IEEE}
}

@article{govender2007review,
  title={A review of hyperspectral remote sensing and its application in vegetation and water resource studies},
  author={Govender, Megandhren and Chetty, Kershani and Bulcock, Hartley},
  journal={Water Sa},
  volume={33},
  number={2},
  pages={145--151},
  year={2007},
  publisher={Water Research Commission (WRC)}
}

@inproceedings{van2004compact,
  title={The Compact High Resolution Imaging Spectrometer (CHRIS): the future of hyperspectral satellite sensors. Imagery of Oostende coastal and inland waters},
  author={Van Mol, Barbara and Ruddick, Kevin and others},
  booktitle={Proceedings of the Airborne Imaging Spectroscopy workshop, Brugge},
  year={2004}
}

@article{vane1993airborne,
  title={The airborne visible/infrared imaging spectrometer (AVIRIS)},
  author={Vane, Gregg and Green, Robert O and Chrien, Thomas G and Enmark, Harry T and Hansen, Earl G and Porter, Wallace M},
  journal={Remote sensing of environment},
  volume={44},
  number={2-3},
  pages={127--143},
  year={1993},
  publisher={Elsevier}
}

@article{GREEN1998227,
title = {Imaging Spectroscopy and the Airborne Visible/Infrared Imaging Spectrometer (AVIRIS)},
journal = {Remote Sensing of Environment},
volume = {65},
number = {3},
pages = {227-248},
year = {1998},
issn = {0034-4257},
doi = {https://doi.org/10.1016/S0034-4257(98)00064-9},
url = {https://www.sciencedirect.com/science/article/pii/S0034425798000649},
author = {Robert O Green, Michael L Eastwood, Charles M Sarture, Thomas G Chrien, Mikael Aronsson, Bruce J Chippendale, Jessica A Faust, Betina E Pavri, Christopher J Chovit, Manuel Solis, Martin R Olah and Orlesa Williams}
}

@INPROCEEDINGS{8127639,
  author={Middleton, Elizabeth M. and Campbell, Petya K.E. and Ong, Lawrence and Landis, David R. and Zhang, Qingyuan and Neigh, Christopher S. and Huemmrich, K. Fred and Ungar, Stephen G and Mandl, Daniel J. and Frye, Stuart W. and Ly, Vuong T. and Cappelaere, Patrice G. and Chien, Steve A. and Franks, Shannon and Pollack, Nathan H.},
  booktitle={2017 IEEE International Geoscience and Remote Sensing Symposium (IGARSS)}, 
  title={Hyperion: The first global orbital spectrometer, earth observing-1 (EO-1) satellite (2000–2017)}, 
  year={2017},
  volume={},
  number={},
  pages={3039-3042},
  doi={10.1109/IGARSS.2017.8127639}}

@article{kruse2003comparison,
  title={Comparison of airborne hyperspectral data and EO-1 Hyperion for mineral mapping},
  author={Kruse, Fred A and Boardman, Joseph W and Huntington, Jonathan F},
  journal={IEEE transactions on Geoscience and Remote Sensing},
  volume={41},
  number={6},
  pages={1388--1400},
  year={2003},
  publisher={IEEE}
}

@inproceedings{galeazzi2008prisma,
  title={The PRISMA program},
  author={Galeazzi, Claudio and Sacchetti, Andrea and Cisbani, Andrea and Babini, Gianni},
  booktitle={IGARSS 2008-2008 IEEE International Geoscience and Remote Sensing Symposium},
  volume={4},
  pages={IV--105},
  year={2008},
  organization={IEEE}
}

@article{lee2013positioning,
  title={Positioning accuracy analysis of KOMPSAT-3 satellite imagery by RPC adjustment},
  author={Lee, Hyoseong and Seo, Doochun and Ahn, Kiweon and Jeong, Dongjang},
  journal={Journal of the Korean Society of Surveying, Geodesy, Photogrammetry and Cartography},
  volume={31},
  number={6\_1},
  pages={503--509},
  year={2013},
  publisher={Korean Society of Surveying, Geodesy, Photogrammetry and Cartography}
}

@inproceedings{kaufmann2012environmental,
  title={The environmental mapping and analysis program (Enmap)},
  author={Kaufmann, Hermann and Segl, Karl and Kuester, Theres and Roga, Christian and Hofer, Stefan and Mueller, Andreas and Chlebek, Christian},
  booktitle={IEEE Int. Geoscience and Remote Sensing Symp},
  year={2012}
}

@article{yokoya2016airborne,
  title={Airborne hyperspectral data over Chikusei},
  author={Yokoya, Naoto and Iwasaki, Akira},
  journal={Space Appl. Lab., Univ. Tokyo, Tokyo, Japan, Tech. Rep. SAL-2016-05-27},
  volume={5},
  year={2016}
}

@article{plaza2009recent,
  title={Recent advances in techniques for hyperspectral image processing},
  author={Plaza, Antonio and Benediktsson, Jon Atli and Boardman, Joseph W and Brazile, Jason and Bruzzone, Lorenzo and Camps-Valls, Gustavo and Chanussot, Jocelyn and Fauvel, Mathieu and Gamba, Paolo and Gualtieri, Anthony and others},
  journal={Remote sensing of environment},
  volume={113},
  pages={S110--S122},
  year={2009},
  publisher={Elsevier}
}

@article{ungar2003overview,
  title={Overview of the earth observing one (EO-1) mission},
  author={Ungar, Stephen G and Pearlman, Jay S and Mendenhall, Jeffrey A and Reuter, Dennis},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={41},
  number={6},
  pages={1149--1159},
  year={2003},
  publisher={IEEE}
}

@inproceedings{nieke2018towards,
  title={Towards the copernicus hyperspectral imaging mission for the environment (CHIME)},
  author={Nieke, Jens and Rast, Michael},
  booktitle={Igarss 2018-2018 ieee international geoscience and remote sensing symposium},
  pages={157--159},
  year={2018},
  organization={IEEE}
}

@article{li2019deep,
  title={Deep learning for hyperspectral image classification: An overview},
  author={Li, Shutao and Song, Weiwei and Fang, Leyuan and Chen, Yushi and Ghamisi, Pedram and Benediktsson, Jon Atli},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={57},
  number={9},
  pages={6690--6709},
  year={2019},
  publisher={IEEE}
}

@article{affonso2017deep,
  title={Deep learning for biological image classification},
  author={Affonso, Carlos and Rossi, Andr{\'e} Luis Debiaso and Vieira, F{\'a}bio Henrique Antunes and de Leon Ferreira, Andr{\'e} Carlos Ponce and others},
  journal={Expert systems with applications},
  volume={85},
  pages={114--122},
  year={2017},
  publisher={Elsevier}
}

@article{minaee2021image,
  title={Image segmentation using deep learning: A survey},
  author={Minaee, Shervin and Boykov, Yuri Y and Porikli, Fatih and Plaza, Antonio J and Kehtarnavaz, Nasser and Terzopoulos, Demetri},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  year={2021},
  publisher={IEEE}
}

@article{tian2020deep,
  title={Deep learning on image denoising: An overview},
  author={Tian, Chunwei and Fei, Lunke and Zheng, Wenxian and Xu, Yong and Zuo, Wangmeng and Lin, Chia-Wen},
  journal={Neural Networks},
  volume={131},
  pages={251--275},
  year={2020},
  publisher={Elsevier}
}

@article{zhao2019object,
  title={Object detection with deep learning: A review},
  author={Zhao, Zhong-Qiu and Zheng, Peng and Xu, Shou-tao and Wu, Xindong},
  journal={IEEE transactions on neural networks and learning systems},
  volume={30},
  number={11},
  pages={3212--3232},
  year={2019},
  publisher={IEEE}
}

@article{voulodimos2018deep,
  title={Deep learning for computer vision: A brief review},
  author={Voulodimos, Athanasios and Doulamis, Nikolaos and Doulamis, Anastasios and Protopapadakis, Eftychios and others},
  journal={Computational intelligence and neuroscience},
  volume={2018},
  year={2018},
  publisher={Hindawi}
}

@article{elharrouss2022backbones,
  title={Backbones-review: Feature extraction networks for deep learning and deep reinforcement learning approaches},
  author={Elharrouss, Omar and Akbari, Younes and Almaadeed, Noor and Al-Maadeed, Somaya},
  journal={arXiv preprint arXiv:2206.08016},
  year={2022}
}

@article{iandola2014densenet,
  title={Densenet: Implementing efficient convnet descriptor pyramids},
  author={Iandola, Forrest and Moskewicz, Matt and Karayev, Sergey and Girshick, Ross and Darrell, Trevor and Keutzer, Kurt},
  journal={arXiv preprint arXiv:1404.1869},
  year={2014}
}

@inproceedings{tan2019efficientnet,
  title={Efficientnet: Rethinking model scaling for convolutional neural networks},
  author={Tan, Mingxing and Le, Quoc},
  booktitle={International conference on machine learning},
  pages={6105--6114},
  year={2019},
  organization={PMLR}
}

@inproceedings{sandler2018mobilenetv2,
  title={Mobilenetv2: Inverted residuals and linear bottlenecks},
  author={Sandler, Mark and Howard, Andrew and Zhu, Menglong and Zhmoginov, Andrey and Chen, Liang-Chieh},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={4510--4520},
  year={2018}
}

@article{hu2015deep,
  title={Deep convolutional neural networks for hyperspectral image classification},
  author={Hu, Wei and Huang, Yangyu and Wei, Li and Zhang, Fan and Li, Hengchao},
  journal={Journal of Sensors},
  volume={2015},
  pages={1--12},
  year={2015},
  publisher={Hindawi Limited}
}

@article{li2018deepunet,
  title={DeepUNet: A deep fully convolutional network for pixel-level sea-land segmentation},
  author={Li, Ruirui and Liu, Wenjie and Yang, Lei and Sun, Shihao and Hu, Wei and Zhang, Fan and Li, Wei},
  journal={IEEE journal of selected topics in applied earth observations and remote sensing},
  volume={11},
  number={11},
  pages={3954--3962},
  year={2018},
  publisher={IEEE}
}

@inproceedings{perazzi2016benchmark,
  title={A benchmark dataset and evaluation methodology for video object segmentation},
  author={Perazzi, Federico and Pont-Tuset, Jordi and McWilliams, Brian and Van Gool, Luc and Gross, Markus and Sorkine-Hornung, Alexander},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={724--732},
  year={2016}
}

@inproceedings{gupta2019lvis,
  title={Lvis: A dataset for large vocabulary instance segmentation},
  author={Gupta, Agrim and Dollar, Piotr and Girshick, Ross},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={5356--5364},
  year={2019}
}

@article{adao2017hyperspectral,
  title={Hyperspectral imaging: A review on UAV-based sensors, data processing and applications for agriculture and forestry},
  author={Ad{\~a}o, Telmo and Hru{\v{s}}ka, Jon{\'a}{\v{s}} and P{\'a}dua, Lu{\'\i}s and Bessa, Jos{\'e} and Peres, Emanuel and Morais, Raul and Sousa, Joaquim Joao},
  journal={Remote sensing},
  volume={9},
  number={11},
  pages={1110},
  year={2017},
  publisher={MDPI}
}

@inproceedings{han2019deep,
  title={Deep residual network of spectral and spatial fusion for hyperspectral image super-resolution},
  author={Han, Xian-Hua and Chen, Yen-Wei},
  booktitle={2019 IEEE Fifth International Conference on Multimedia Big Data (BigMM)},
  pages={266--270},
  year={2019},
  organization={IEEE}
}

@article{hu2020pan,
  title={Pan-sharpening via multiscale dynamic convolutional neural network},
  author={Hu, Jianwen and Hu, Pei and Kang, Xudong and Zhang, Hui and Fan, Shaosheng},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={59},
  number={3},
  pages={2231--2244},
  year={2020},
  publisher={IEEE}
}

@article{chen2021hyperspectral,
  title={Hyperspectral image super-resolution with self-supervised spectral-spatial residual network},
  author={Chen, Wenjing and Zheng, Xiangtao and Lu, Xiaoqiang},
  journal={Remote Sensing},
  volume={13},
  number={7},
  pages={1260},
  year={2021},
  publisher={MDPI}
}

@inproceedings{zhang2021survey,
  title={A survey of hyperspectral image super-resolution technology},
  author={Zhang, Meilin and Sun, Xiongli and Zhu, Qiqi and Zheng, Guizhou},
  booktitle={2021 IEEE International Geoscience and Remote Sensing Symposium IGARSS},
  pages={4476--4479},
  year={2021},
  organization={IEEE}
}

@article{purushwalkam2020demystifying,
  title={Demystifying contrastive self-supervised learning: Invariances, augmentations and dataset biases},
  author={Purushwalkam, Senthil and Gupta, Abhinav},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={3407--3418},
  year={2020}
}

@article{jaiswal2020survey,
  title={A survey on contrastive self-supervised learning},
  author={Jaiswal, Ashish and Babu, Ashwin Ramesh and Zadeh, Mohammad Zaki and Banerjee, Debapriya and Makedon, Fillia},
  journal={Technologies},
  volume={9},
  number={1},
  pages={2},
  year={2020},
  publisher={MDPI}
}

@article{robinson2020contrastive,
  title={Contrastive learning with hard negative samples},
  author={Robinson, Joshua and Chuang, Ching-Yao and Sra, Suvrit and Jegelka, Stefanie},
  journal={arXiv preprint arXiv:2010.04592},
  year={2020}
}

@inproceedings{chen2020simple,
  title={A simple framework for contrastive learning of visual representations},
  author={Chen, Ting and Kornblith, Simon and Norouzi, Mohammad and Hinton, Geoffrey},
  booktitle={International conference on machine learning},
  pages={1597--1607},
  year={2020},
  organization={PMLR}
}

@article{qian2021hyperspectral,
  title={Hyperspectral satellites, evolution, and development history},
  author={Qian, Shen-En},
  journal={IEEE Journal of Selected Topics in Applied Earth Observations and Remote Sensing},
  volume={14},
  pages={7032--7056},
  year={2021},
  publisher={IEEE}
}

@misc { PURR1947,
	title = {220 Band AVIRIS Hyperspectral Image Data Set: June 12, 1992 Indian Pine Test Site 3},
	month = {Sep},
	url = {https://purr.purdue.edu/publications/1947/1},
	year = {2015},
	doi = {doi:/10.4231/R7RX991C},
	author = {Marion F. Baumgardner , and Larry L. Biehl , and David A. Landgrebe ,}
}

@inproceedings{kunkel1988rosis,
  title={ROSIS (Reflective Optics System Imaging Spectrometer)-A candidate instrument for polar platform missions},
  author={Kunkel, B and Blechinger, F and Lutz, R and Doerffer, R and Van der Piepen, H and Schroder, M},
  booktitle={Optoelectronic technologies for remote sensing from space},
  volume={868},
  pages={134--141},
  year={1988},
  organization={SPIE}
}

@conference{chakrabarti2011statistics,
  title={{Statistics of Real-World Hyperspectral Images}},
  author={Chakrabarti, A. and Zickler, T.},
  booktitle={Proc.~IEEE Conf.~on Computer Vision and Pattern Recognition (CVPR)},
  pages={193--200},
  year={2011}
}

@article{article,
author = {Kang, Xudong and Li, Shutao and Fang, Leyuan and Li, Meixiu and Benediktsson, Jon},
year = {2015},
month = {01},
pages = {},
title = {Extended Random Walker-Based Classification of Hyperspectral Images},
volume = {53},
journal = {IEEE Transactions on Geoscience and Remote Sensing},
doi = {10.1109/TGRS.2014.2319373}
}

@article{article2,
author = {Zhou, Xiong and Prasad, Saurabh},
year = {2017},
month = {09},
pages = {1-1},
title = {Domain Adaptation for Robust Classification of Disparate Hyperspectral Images},
volume = {PP},
journal = {IEEE Transactions on Computational Imaging},
doi = {10.1109/TCI.2017.2752150}
}

@article{he2021spatial,
  title={Spatial-spectral transformer for hyperspectral image classification},
  author={He, Xin and Chen, Yushi and Lin, Zhouhan},
  journal={Remote Sensing},
  volume={13},
  number={3},
  pages={498},
  year={2021},
  publisher={MDPI}
}

@article{tan2021deep,
  title={Deep global-local transformer network combined with extended morphological profiles for hyperspectral image classification},
  author={Tan, Xiong and Gao, Kuiliang and Liu, Bing and Fu, Yumeng and Kang, Lei},
  journal={Journal of Applied Remote Sensing},
  volume={15},
  number={3},
  pages={038509--038509},
  year={2021},
  publisher={Society of Photo-Optical Instrumentation Engineers}
}

@article{dang2023double,
  title={Double-branch feature fusion transformer for hyperspectral image classification},
  author={Dang, Lanxue and Weng, Libo and Hou, Yane and Zuo, Xianyu and Liu, Yang},
  journal={Scientific Reports},
  volume={13},
  number={1},
  pages={272},
  year={2023},
  publisher={Nature Publishing Group UK London}
}

@inproceedings{ducay2022hyperspectral,
  title={Hyperspectral-multispectral image fusion using nearest-neighbor diffusion-based sharpening algorithm},
  author={Ducay, Rey and Messinger, David W},
  booktitle={Algorithms, Technologies, and Applications for Multispectral and Hyperspectral Imaging XXVIII},
  volume={12094},
  pages={213--225},
  year={2022},
  organization={SPIE}
}

@inproceedings{polk2022unsupervised,
  title={Unsupervised detection of ash dieback disease (Hymenoscyphus fraxineus) using diffusion-based hyperspectral image clustering},
  author={Polk, Sam L and Chan, Aland HY and Cui, Kangning and Plemmons, Robert J and Coomes, David A and Murphy, James M},
  booktitle={IGARSS 2022-2022 IEEE International Geoscience and Remote Sensing Symposium},
  pages={2287--2290},
  year={2022},
  organization={IEEE}
}

@article{miao2023dds2m,
  title={DDS2M: Self-Supervised Denoising Diffusion Spatio-Spectral Model for Hyperspectral Image Restoration},
  author={Miao, Yuchun and Zhang, Lefei and Zhang, Liangpei and Tao, Dacheng},
  journal={arXiv preprint arXiv:2303.06682},
  year={2023}
}

@article{mughees2018multiple,
  title={Multiple deep-belief-network-based spectral-spatial classification of hyperspectral images},
  author={Mughees, Atif and Tao, Linmi},
  journal={Tsinghua Science and Technology},
  volume={24},
  number={2},
  pages={183--194},
  year={2018},
  publisher={TUP}
}

@article{ortega2019use,
  title={Use of hyperspectral/multispectral imaging in gastroenterology. Shedding some--different--light into the dark},
  author={Ortega, Samuel and Fabelo, Himar and Iakovidis, Dimitris K and Koulaouzidis, Anastasios and Callico, Gustavo M},
  journal={Journal of clinical medicine},
  volume={8},
  number={1},
  pages={36},
  year={2019},
  publisher={MDPI}
}


@article{li2022manifold,
  title={Manifold-Based Multi-Deep Belief Network for Feature Extraction of Hyperspectral Image},
  author={Li, Zhengying and Huang, Hong and Zhang, Zhen and Shi, Guangyao},
  journal={Remote Sensing},
  volume={14},
  number={6},
  pages={1484},
  year={2022},
  publisher={MDPI}
}

@inproceedings{cheng2019prospect,
  title={Prospect of application of hyperspectral imaging technology in public security},
  author={Cheng, Cheng and Zhao, Bo},
  booktitle={International Conference on Applications and Techniques in Cyber Security and Intelligence ATCI 2018: Applications and Techniques in Cyber Security and Intelligence},
  pages={299--304},
  year={2019},
  organization={Springer}
}

@article{brisco1998precision,
  title={Precision agriculture and the role of remote sensing: a review},
  author={Brisco, B and Brown, RJ and Hirose, T and McNairn, H and Staenz, K},
  journal={Canadian Journal of Remote Sensing},
  volume={24},
  number={3},
  pages={315--327},
  year={1998},
  publisher={Taylor \& Francis}
}

@article{maes2019perspectives,
  title={Perspectives for remote sensing with unmanned aerial vehicles in precision agriculture},
  author={Maes, Wouter H and Steppe, Kathy},
  journal={Trends in plant science},
  volume={24},
  number={2},
  pages={152--164},
  year={2019},
  publisher={Elsevier}
}

@article{bienkowski2019detection,
  title={Detection and differentiation between potato (Solanum tuberosum) diseases using calibration models trained with non-imaging spectrometry data},
  author={Bienkowski, Damian and Aitkenhead, Matt J and Lees, Alison K and Gallagher, Christopher and Neilson, Roy},
  journal={Computers and Electronics in Agriculture},
  volume={167},
  pages={105056},
  year={2019},
  publisher={Elsevier}
}

@article{adam2010multispectral,
  title={Multispectral and hyperspectral remote sensing for identification and mapping of wetland vegetation: a review},
  author={Adam, Elhadi and Mutanga, Onisimo and Rugege, Denis},
  journal={Wetlands ecology and management},
  volume={18},
  pages={281--296},
  year={2010},
  publisher={Springer}
}

@article{rasti2018noise,
  title={Noise reduction in hyperspectral imagery: Overview and application},
  author={Rasti, Behnood and Scheunders, Paul and Ghamisi, Pedram and Licciardi, Giorgio and Chanussot, Jocelyn},
  journal={Remote Sensing},
  volume={10},
  number={3},
  pages={482},
  year={2018},
  publisher={MDPI}
}

@article{lecun1998gradient,
  title={Gradient-based learning applied to document recognition},
  author={LeCun, Yann and Bottou, L{\'e}on and Bengio, Yoshua and Haffner, Patrick},
  journal={Proceedings of the IEEE},
  volume={86},
  number={11},
  pages={2278--2324},
  year={1998},
  publisher={Ieee}
}

@article{krizhevsky2017imagenet,
  title={Imagenet classification with deep convolutional neural networks},
  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  journal={Communications of the ACM},
  volume={60},
  number={6},
  pages={84--90},
  year={2017},
  publisher={AcM New York, NY, USA}
}

@article{howard2017mobilenets,
  title={Mobilenets: Efficient convolutional neural networks for mobile vision applications},
  author={Howard, Andrew G and Zhu, Menglong and Chen, Bo and Kalenichenko, Dmitry and Wang, Weijun and Weyand, Tobias and Andreetto, Marco and Adam, Hartwig},
  journal={arXiv preprint arXiv:1704.04861},
  year={2017}
}

@article{gao2021deep,
  title={Deep Transformer Network for Hyperspectral Image Classification},
  author={Gao, Kuiliang and Liu, Bing and Xue, Zhixiang and Zuo, Xibing and Sun, Yifan and Dai, Mofan and others},
  journal={Academic Journal of Computing \& Information Science},
  volume={4},
  number={7},
  pages={11--17},
  year={2021},
  publisher={Francis Academic Press}
}

@article{huang20223,
  title={A 3-d-swin transformer-based hierarchical contrastive learning method for hyperspectral image classification},
  author={Huang, Xin and Dong, Mengjie and Li, Jiayi and Guo, Xian},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={60},
  pages={1--15},
  year={2022},
  publisher={IEEE}
}

@article{kipf2016semi,
  title={Semi-supervised classification with graph convolutional networks},
  author={Kipf, Thomas N and Welling, Max},
  journal={arXiv preprint arXiv:1609.02907},
  year={2016}
}

@inproceedings{tong2020few,
  title={Few-shot learning with attention-weighted graph convolutional networks for hyperspectral image classification},
  author={Tong, Xinyi and Yin, Jihao and Han, Bingnan and Qv, Hui},
  booktitle={2020 IEEE International Conference on Image Processing (ICIP)},
  pages={1686--1690},
  year={2020},
  organization={IEEE}
}

@article{yan2022pansharpening,
  title={When pansharpening meets graph convolution network and knowledge distillation},
  author={Yan, Keyu and Zhou, Man and Liu, Liu and Xie, Chengjun and Hong, Danfeng},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={60},
  pages={1--15},
  year={2022},
  publisher={IEEE}
}

@article{cai2020remote,
  title={Remote sensing image classification based on a cross-attention mechanism and graph convolution},
  author={Cai, Weiwei and Wei, Zhanguo},
  journal={IEEE Geoscience and Remote Sensing Letters},
  volume={19},
  pages={1--5},
  year={2020},
  publisher={IEEE}
}

@inproceedings{jia2022mutual,
  title={Mutual learning graph convolutional network for hyperspectral image classification},
  author={Jia, ChaoJie and Zhan, Kun},
  booktitle={International Conference on Cloud Computing, Performance Computing, and Deep Learning (CCPCDL 2022)},
  volume={12287},
  pages={338--344},
  year={2022},
  organization={SPIE}
}

@article{sabour2017dynamic,
  title={Dynamic routing between capsules},
  author={Sabour, Sara and Frosst, Nicholas and Hinton, Geoffrey E},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@article{yin2019hyperspectral,
  title={Hyperspectral image classification using CapsNet with well-initialized shallow layers},
  author={Yin, Jihao and Li, Sen and Zhu, Hongmei and Luo, Xiaoyan},
  journal={IEEE Geoscience and Remote Sensing Letters},
  volume={16},
  number={7},
  pages={1095--1099},
  year={2019},
  publisher={IEEE}
}

@article{jiang2020hyperspectral,
  title={Hyperspectral image classification with CapsNet and Markov random fields},
  author={Jiang, Xuefeng and Zhang, Yue and Liu, Wenbo and Gao, Junyu and Liu, Junrui and Zhang, Yanning and Lin, Jianzhe},
  journal={IEEE Access},
  volume={8},
  pages={191956--191968},
  year={2020},
  publisher={IEEE}
}

@article{shi2023multi,
  title={A multi-scale residual capsule network for hyperspectral image classification with small training samples},
  author={Shi, Meilin and Zeng, Xilong and Ren, Jiansi and Shi, Yichang},
  journal={Multimedia Tools and Applications},
  pages={1--29},
  year={2023},
  publisher={Springer}
}

@article{shu2023res,
  title={RES-CapsNet: an improved capsule network for micro-expression recognition},
  author={Shu, Xin and Li, Jia and Shi, Liang and Huang, Shucheng},
  journal={Multimedia Systems},
  pages={1--9},
  year={2023},
  publisher={Springer}
}

@article{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@article{dosovitskiy2020image,
  title={An image is worth 16x16 words: Transformers for image recognition at scale},
  author={Dosovitskiy, Alexey and Beyer, Lucas and Kolesnikov, Alexander and Weissenborn, Dirk and Zhai, Xiaohua and Unterthiner, Thomas and Dehghani, Mostafa and Minderer, Matthias and Heigold, Georg and Gelly, Sylvain and others},
  journal={arXiv preprint arXiv:2010.11929},
  year={2020}
}

@article{ulrichsen2023operational,
  title={Operational Neural Networks for Efficient Hyperspectral Single-Image Super-Resolution},
  author={Ulrichsen, Alexander and Murray, Paul and Marshall, Stephen and Gabbouj, Moncef and Kiranyaz, Serkan and Yamac, Mehmet and Aburaed, Nour},
  journal={arXiv preprint arXiv:2303.16636},
  year={2023}
}

@article{qu2023sub,
  title={A sub-pixel convolution-based improved bidirectional feature pyramid network for pansharpening},
  author={Qu, Jiantao and Yin, Junru and Jiang, Yuhao and Huang, Wei and Chen, Qiqiang},
  journal={Remote Sensing Letters},
  volume={14},
  number={1},
  pages={91--101},
  year={2023},
  publisher={Taylor \& Francis}
}

@article{cao2023ddrf,
  title={DDRF: Denoising Diffusion Model for Remote Sensing Image Fusion},
  author={Cao, ZiHan and Cao, ShiQi and Wu, Xiao and Hou, JunMing and Ran, Ran and Deng, Liang-Jian},
  journal={arXiv preprint arXiv:2304.04774},
  year={2023}
}

@article{liu2023pansharpening,
  title={Pansharpening Model of Transferable Remote Sensing Images Based on Feature Fusion and Attention Modules},
  author={Liu, Hui and Deng, Liangfeng and Dou, Yibo and Zhong, Xiwu and Qian, Yurong},
  journal={Sensors},
  volume={23},
  number={6},
  pages={3275},
  year={2023},
  publisher={MDPI}
}

@article{qiao2023hmft,
  title={HMFT: Hyperspectral and Multispectral Image Fusion Super-Resolution Method Based on Efficient Transformer and Spatial-Spectral Attention Mechanism},
  author={Qiao, Baojun and Xu, Binghui and Xie, Yi and Lin, Yinghao and Liu, Yang and Zuo, Xianyu and others},
  journal={Computational Intelligence and Neuroscience},
  volume={2023},
  year={2023},
  publisher={Hindawi}
}

@article{wang2023mct,
  title={MCT-Net: Multi-hierarchical cross transformer for hyperspectral and multispectral image fusion},
  author={Wang, Xianghai and Wang, Xinying and Song, Ruoxi and Zhao, Xiaoyang and Zhao, Keyun},
  journal={Knowledge-Based Systems},
  volume={264},
  pages={110362},
  year={2023},
  publisher={Elsevier}
}

@article{ding2023multi,
  title={Multi-scale Receptive Fields: Graph Attention Neural Network for Hyperspectral Image Classification},
  author={Ding, Yao and Zhang, Zhili and Zhao, Xiaofeng and Hong, Danfeng and Cai, Wei and Yang, Nengjun and Wang, Bei},
  journal={Expert Systems with Applications},
  pages={119858},
  year={2023},
  publisher={Elsevier}
}

@article{azarang2023spectral,
  title={Spectral unmixing of hyperspectral images based on block sparse structure},
  author={Azarang, Seyed Hossein Mosavi and Rajabi, Roozbeh and Zayyani, Hadi and Zehtabian, Amin},
  journal={Journal of Applied Remote Sensing},
  volume={17},
  number={1},
  pages={016510},
  year={2023},
  publisher={SPIE}
}

@article{fang2023nonlinear,
  title={Nonlinear Hyperspectral Unmixing based on Multilinear Mixing Model using Convolutional Autoencoders},
  author={Fang, Tingting and Zhu, Fei and Chen, Jie},
  journal={arXiv preprint arXiv:2303.08156},
  year={2023}
}

@article{sun2023sislu,
  title={SISLU-Net: Spatial Information-Assisted Spectral Information Learning Unmixing Network for Hyperspectral Images},
  author={Sun, Le and Chen, Ying and Li, Baozhu},
  journal={Remote Sensing},
  volume={15},
  number={3},
  pages={817},
  year={2023},
  publisher={MDPI}
}

@article{li2023attention,
  title={An Attention-Based 3D Convolutional Autoencoder for Few-Shot Hyperspectral Unmixing and Classification},
  author={Li, Chunyu and Cai, Rong and Yu, Junchuan},
  journal={Remote Sensing},
  volume={15},
  number={2},
  pages={451},
  year={2023},
  publisher={MDPI}
}

@article{ran2023guidednet,
  title={GuidedNet: A General CNN Fusion Framework via High-Resolution Guidance for Hyperspectral Image Super-Resolution},
  author={Ran, Ran and Deng, Liang-Jian and Jiang, Tai-Xiang and Hu, Jin-Fan and Chanussot, Jocelyn and Vivone, Gemine},
  journal={IEEE Transactions on Cybernetics},
  year={2023},
  publisher={IEEE}
}

@inproceedings{yu2023dstrans,
  title={DSTrans: Dual-Stream Transformer for Hyperspectral Image Restoration},
  author={Yu, Dabing and Li, Qingwu and Wang, Xiaolin and Zhang, Zhiliang and Qian, Yixi and Xu, Chang},
  booktitle={Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision},
  pages={3739--3749},
  year={2023}
}

@article{zou2023hyperspectral,
  title={Hyperspectral image super-resolution using cluster-based deep convolutional networks},
  author={Zou, Changzhong and Zhang, Can},
  journal={Signal Processing: Image Communication},
  volume={110},
  pages={116884},
  year={2023},
  publisher={Elsevier}
}

@article{xiu2023cot,
  title={CoT-MISR: Marrying Convolution and Transformer for Multi-Image Super-Resolution},
  author={Xiu, Mingming and Nie, Yang and Song, Qing and Liu, Chun},
  journal={arXiv preprint arXiv:2303.06548},
  year={2023}
}

@article{hu2022fusformer,
  title={Fusformer: A transformer-based fusion network for hyperspectral image super-resolution},
  author={Hu, Jin-Fan and Huang, Ting-Zhu and Deng, Liang-Jian and Dou, Hong-Xia and Hong, Danfeng and Vivone, Gemine},
  journal={IEEE Geoscience and Remote Sensing Letters},
  volume={19},
  pages={1--5},
  year={2022},
  publisher={IEEE}
}

@article{liang2023multi,
  title={Multi-scale hybrid attention graph convolution neural network for remote sensing images super-resolution},
  author={Liang, Guojun and Kintak, U and Yin, Haichang and Liu, Jin and Luo, Huibin},
  journal={Signal Processing},
  volume={207},
  pages={108954},
  year={2023},
  publisher={Elsevier}
}

@article{li2023sd,
  title={SD-CapsNet: A Siamese Dense Capsule Network for SAR Image Registration with Complex Scenes},
  author={Li, Bangjie and Guan, Dongdong and Zheng, Xiaolong and Chen, Zhengsheng and Pan, Lefei},
  journal={Remote Sensing},
  volume={15},
  number={7},
  pages={1871},
  year={2023},
  publisher={MDPI}
}

@article{ren2022hyperspectral,
  title={Hyperspectral image classification using multi-level features fusion capsule network with a dense structure},
  author={Ren, Jiansi and Shi, Meilin and Chen, Jiannan and Wang, Ruoxiang and Wang, Xin},
  journal={Applied Intelligence},
  pages={1--20},
  year={2022},
  publisher={Springer}
}

@article{liu2023sifnet,
  title={SIFNet: A self-attention interaction fusion network for multisource satellite imagery template matching},
  author={Liu, Ming and Zhou, Gaoxiang and Ma, Lingfei and Li, Liangzhi and Mei, Qiong},
  journal={International Journal of Applied Earth Observation and Geoinformation},
  volume={118},
  pages={103247},
  year={2023},
  publisher={Elsevier}
}

@article{zhang2023image,
  title={Image Registration Algorithm for Remote Sensing Images Based on Pixel Location Information},
  author={Zhang, Xuming and Zhou, Yao and Qiao, Peng and Lv, Xiaoning and Li, Jimin and Du, Tianyu and Cai, Yiming},
  journal={Remote Sensing},
  volume={15},
  number={2},
  pages={436},
  year={2023},
  publisher={MDPI}
}

@inproceedings{pankaj2023robust,
  title={A Robust Estimation Method for Automatic Registration of Remote Sensing Imagery},
  author={Pankaj, Dhanya S and Nidamanuri, Rama Rao},
  booktitle={2023 International Conference on Machine Intelligence for GeoAnalytics and Remote Sensing (MIGARS)},
  volume={1},
  pages={1--4},
  year={2023},
  organization={IEEE}
}

@article{qureshi2019hyperspectral,
  title={Hyperspectral document image processing: Applications, challenges and future prospects},
  author={Qureshi, Rizwan and Uzair, Muhammad and Khurshid, Khurram and Yan, Hong},
  journal={Pattern Recognition},
  volume={90},
  pages={12--22},
  year={2019},
  publisher={Elsevier}
}

@article{mansfield2014multispectral,
  title={Multispectral imaging: a review of its technical aspects and applications in anatomic pathology},
  author={Mansfield, JR},
  journal={Veterinary pathology},
  volume={51},
  number={1},
  pages={185--210},
  year={2014},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{priya2022hyperspectral,
  title={Hyperspectral and Multispectral Image Fusion Using Deep Convolutional Neural Network-ResNet Fusion},
  author={Priya, K and Rajkumar, KK},
  year={2022},
  publisher={IntechOpen}
}

@article{gao2022hyperspectral,
  title={Hyperspectral and Multispectral Image Fusion Via Self-Supervised Loss and Separable Loss},
  author={Gao, Huiling and Li, Shutao and Dian, Renwei},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={60},
  pages={1--12},
  year={2022},
  publisher={IEEE}
}

@article{sun2022mlr,
  title={MLR-DBPFN: A multi-scale low rank deep back projection fusion network for anti-noise hyperspectral and multispectral image fusion},
  author={Sun, Weiwei and Ren, Kai and Meng, Xiangchao and Yang, Gang and Xiao, Chenchao and Peng, Jiangtao and Huang, Jingfeng},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={60},
  pages={1--14},
  year={2022},
  publisher={IEEE}
}

@article{palsson2017multispectral,
  title={Multispectral and hyperspectral image fusion using a 3-D-convolutional neural network},
  author={Palsson, Frosti and Sveinsson, Johannes R and Ulfarsson, Magnus O},
  journal={IEEE Geoscience and Remote Sensing Letters},
  volume={14},
  number={5},
  pages={639--643},
  year={2017},
  publisher={IEEE}
}

@article{zhou2020perceppan,
  title={PercepPan: Towards unsupervised pan-sharpening based on perceptual loss},
  author={Zhou, Changsheng and Zhang, Jiangshe and Liu, Junmin and Zhang, Chunxia and Fei, Rongrong and Xu, Shuang},
  journal={Remote Sensing},
  volume={12},
  number={14},
  pages={2318},
  year={2020},
  publisher={MDPI}
}

@article{li2020hyperspectral,
  title={Hyperspectral image super-resolution by band attention through adversarial learning},
  author={Li, Jiaojiao and Cui, Ruxing and Li, Bo and Song, Rui and Li, Yunsong and Dai, Yuchao and Du, Qian},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={58},
  number={6},
  pages={4304--4318},
  year={2020},
  publisher={IEEE}
}

@article{jaiswal2021critical,
  title={Critical insights into modern hyperspectral image applications through deep learning},
  author={Jaiswal, Garima and Sharma, Arun and Yadav, Sumit Kumar},
  journal={Wiley Interdisciplinary Reviews: Data Mining and Knowledge Discovery},
  volume={11},
  number={6},
  pages={e1426},
  year={2021},
  publisher={Wiley Online Library}
}

@article{wang2023ssanet,
  title={SSANet: An Adaptive Spectral--Spatial Attention Autoencoder Network for Hyperspectral Unmixing},
  author={Wang, Jie and Xu, Jindong and Chong, Qianpeng and Liu, Zhaowei and Yan, Weiqing and Xing, Haihua and Xing, Qianguo and Ni, Mengying},
  journal={Remote Sensing},
  volume={15},
  number={8},
  pages={2070},
  year={2023},
  publisher={MDPI}
}

@article{yu2017convolutional,
  title={Convolutional neural networks for hyperspectral image classification},
  author={Yu, Shiqi and Jia, Sen and Xu, Chunyan},
  journal={Neurocomputing},
  volume={219},
  pages={88--98},
  year={2017},
  publisher={Elsevier}
}

@article{liu2023multi,
  title={Multi-Dataset Hyper-CNN for Hyperspectral Image Segmentation of Remote Sensing Images},
  author={Liu, Li and Awwad, Emad Mahrous and Ali, Yasser A and Al-Razgan, Muna and Maarouf, Ali and Abualigah, Laith and Hoshyar, Azadeh Noori},
  journal={Processes},
  volume={11},
  number={2},
  pages={435},
  year={2023},
  publisher={MDPI}
}

@article{chhapariya2022cnn,
  title={CNN-Based Salient Object Detection on Hyperspectral Images Using Extended Morphology},
  author={Chhapariya, Koushikey and Buddhiraju, Krishna Mohan and Kumar, Anil},
  journal={IEEE Geoscience and Remote Sensing Letters},
  volume={19},
  pages={1--5},
  year={2022},
  publisher={IEEE}
}

@article{rangnekar2020aerorit,
  title={Aerorit: A new scene for hyperspectral image analysis},
  author={Rangnekar, Aneesh and Mokashi, Nilay and Ientilucci, Emmett J and Kanan, Christopher and Hoffman, Matthew J},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={58},
  number={11},
  pages={8116--8124},
  year={2020},
  publisher={IEEE}
}

@article{paoletti2018new,
  title={A new deep convolutional neural network for fast hyperspectral image classification},
  author={Paoletti, Mercedes E and Haut, Juan Mario and Plaza, Javier and Plaza, Antonio},
  journal={ISPRS journal of photogrammetry and remote sensing},
  volume={145},
  pages={120--147},
  year={2018},
  publisher={Elsevier}
}

@article{yu2020simplified,
  title={A simplified 2D-3D CNN architecture for hyperspectral image classification based on spatial--spectral fusion},
  author={Yu, Chunyan and Han, Rui and Song, Meiping and Liu, Caiyu and Chang, Chein-I},
  journal={IEEE Journal of Selected Topics in Applied Earth Observations and Remote Sensing},
  volume={13},
  pages={2485--2501},
  year={2020},
  publisher={IEEE}
}

@article{wu2020three,
  title={Three-dimensional resnext network using feature fusion and label smoothing for hyperspectral image classification},
  author={Wu, Peida and Cui, Ziguan and Gan, Zongliang and Liu, Feng},
  journal={Sensors},
  volume={20},
  number={6},
  pages={1652},
  year={2020},
  publisher={MDPI}
}

@article{jing2020self,
  title={Self-supervised visual feature learning with deep neural networks: A survey},
  author={Jing, Longlong and Tian, Yingli},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={43},
  number={11},
  pages={4037--4058},
  year={2020},
  publisher={IEEE}
}

@article{zhao2020semi,
  title={Semi-supervised broad learning system based on manifold regularization and broad network},
  author={Zhao, Huimin and Zheng, Jianjie and Deng, Wu and Song, Yingjie},
  journal={IEEE Transactions on Circuits and Systems I: Regular Papers},
  volume={67},
  number={3},
  pages={983--994},
  year={2020},
  publisher={IEEE}
}

@article{sonderby2016ladder,
  title={Ladder variational autoencoders},
  author={S{\o}nderby, Casper Kaae and Raiko, Tapani and Maal{\o}e, Lars and S{\o}nderby, S{\o}ren Kaae and Winther, Ole},
  journal={Advances in neural information processing systems},
  volume={29},
  year={2016}
}

@article{kingma2013auto,
  title={Auto-encoding variational bayes},
  author={Kingma, Diederik P and Welling, Max},
  journal={arXiv preprint arXiv:1312.6114},
  year={2013}
}

@article{goodfellow2014generative,
  title={Generative adversarial nets Advances in neural information processing systems},
  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1406.2661},
  year={2014}
}

@inproceedings{khan2018adversarial,
  title={Adversarial training of variational auto-encoders for high fidelity image generation},
  author={Khan, Salman H and Hayat, Munawar and Barnes, Nick},
  booktitle={2018 IEEE winter conference on applications of computer vision (WACV)},
  pages={1312--1320},
  year={2018},
  organization={IEEE}
}

@article{krsynthesis,
  title={Synthesis of Image from Text using Generative Adversarial Networks},
  author={KR, Remya and Jayasree, M}
}

@inproceedings{karnewar2020msg,
  title={Msg-gan: Multi-scale gradients for generative adversarial networks},
  author={Karnewar, Animesh and Wang, Oliver},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={7799--7808},
  year={2020}
}

@inproceedings{kurach2019large,
  title={A large-scale study on regularization and normalization in GANs},
  author={Kurach, Karol and Lu{\v{c}}i{\'c}, Mario and Zhai, Xiaohua and Michalski, Marcin and Gelly, Sylvain},
  booktitle={International conference on machine learning},
  pages={3581--3590},
  year={2019},
  organization={PMLR}
}

@article{nguyen2017dual,
  title={Dual discriminator generative adversarial nets},
  author={Nguyen, Tu and Le, Trung and Vu, Hung and Phung, Dinh},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@article{oord2018representation,
  title={Representation learning with contrastive predictive coding},
  author={Oord, Aaron van den and Li, Yazhe and Vinyals, Oriol},
  journal={arXiv preprint arXiv:1807.03748},
  year={2018}
}

@inproceedings{wu2018unsupervised,
  title={Unsupervised feature learning via non-parametric instance discrimination},
  author={Wu, Zhirong and Xiong, Yuanjun and Yu, Stella X and Lin, Dahua},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={3733--3742},
  year={2018}
}

@article{hjelm2018learning,
  title={Learning deep representations by mutual information estimation and maximization},
  author={Hjelm, R Devon and Fedorov, Alex and Lavoie-Marchildon, Samuel and Grewal, Karan and Bachman, Phil and Trischler, Adam and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1808.06670},
  year={2018}
}

@inproceedings{he2020momentum,
  title={Momentum contrast for unsupervised visual representation learning},
  author={He, Kaiming and Fan, Haoqi and Wu, Yuxin and Xie, Saining and Girshick, Ross},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={9729--9738},
  year={2020}
}

@article{hou2021hyperspectral,
  title={Hyperspectral imagery classification based on contrastive learning},
  author={Hou, Sikang and Shi, Hongye and Cao, Xianghai and Zhang, Xiaohua and Jiao, Licheng},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={60},
  pages={1--13},
  year={2021},
  publisher={IEEE}
}

@article{khan2020survey,
  title={A survey of the recent architectures of deep convolutional neural networks},
  author={Khan, Asifullah and Sohail, Anabia and Zahoora, Umme and Qureshi, Aqsa Saeed},
  journal={Artificial intelligence review},
  volume={53},
  pages={5455--5516},
  year={2020},
  publisher={Springer}
}

@inproceedings{wald2000quality,
  title={Quality of high resolution synthesised images: Is there a simple criterion?},
  author={Wald, Lucien},
  booktitle={Third conference" Fusion of Earth data: merging point measurements, raster maps and remotely sensed images"},
  pages={99--103},
  year={2000},
  organization={SEE/URISCA}
}

@article{yokoya2011coupled,
  title={Coupled nonnegative matrix factorization unmixing for hyperspectral and multispectral data fusion},
  author={Yokoya, Naoto and Yairi, Takehisa and Iwasaki, Akira},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={50},
  number={2},
  pages={528--537},
  year={2011},
  publisher={IEEE}
}

@article{zheng2020hyperspectral,
  title={Hyperspectral pansharpening using deep prior and dual attention residual network},
  author={Zheng, Yuxuan and Li, Jiaojiao and Li, Yunsong and Guo, Jie and Wu, Xianyun and Chanussot, Jocelyn},
  journal={IEEE transactions on geoscience and remote sensing},
  volume={58},
  number={11},
  pages={8059--8076},
  year={2020},
  publisher={IEEE}
}

@article{bandara2021hyperspectral,
  title={Hyperspectral pansharpening based on improved deep image prior and residual reconstruction},
  author={Bandara, Wele Gedara Chaminda and Valanarasu, Jeya Maria Jose and Patel, Vishal M},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={60},
  pages={1--16},
  year={2021},
  publisher={IEEE}
}

@article{ge2020learning,
  title={A learning-enhanced two-pair spatiotemporal reflectance fusion model for GF-2 and GF-1 WFV satellite data},
  author={Ge, Yanqin and Li, Yanrong and Chen, Jinyong and Sun, Kang and Li, Dacheng and Han, Qijin},
  journal={Sensors},
  volume={20},
  number={6},
  pages={1789},
  year={2020},
  publisher={MDPI}
}

@article{simoes2014convex,
  title={A convex formulation for hyperspectral image superresolution via subspace-based regularization},
  author={Simoes, Miguel and Bioucas-Dias, Jos{\'e} and Almeida, Luis B and Chanussot, Jocelyn},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={53},
  number={6},
  pages={3373--3388},
  year={2014},
  publisher={IEEE}
}

@inproceedings{yang2017pannet,
  title={PanNet: A deep network architecture for pan-sharpening},
  author={Yang, Junfeng and Fu, Xueyang and Hu, Yuwen and Huang, Yue and Ding, Xinghao and Paisley, John},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={5449--5457},
  year={2017}
}

@inproceedings{lee2021sipsa,
  title={Sipsa-net: Shift-invariant pan sharpening with moving object alignment for satellite imagery},
  author={Lee, Jaehyup and Seo, Soomin and Kim, Munchurl},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={10166--10174},
  year={2021}
}

@inproceedings{xu2021deep,
  title={Deep gradient projection networks for pan-sharpening},
  author={Xu, Shuang and Zhang, Jiangshe and Zhao, Zixiang and Sun, Kai and Liu, Junmin and Zhang, Chunxia},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={1366--1375},
  year={2021}
}

@inproceedings{schroff2015facenet,
  title={Facenet: A unified embedding for face recognition and clustering},
  author={Schroff, Florian and Kalenichenko, Dmitry and Philbin, James},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={815--823},
  year={2015}
}

@inproceedings{hadsell2006dimensionality,
  title={Dimensionality reduction by learning an invariant mapping},
  author={Hadsell, Raia and Chopra, Sumit and LeCun, Yann},
  booktitle={2006 IEEE Computer Society Conference on Computer Vision and Pattern Recognition (CVPR'06)},
  volume={2},
  pages={1735--1742},
  year={2006},
  organization={IEEE}
}

@article{collado2022comprehensive,
  title={Comprehensive study of good model training for prostate segmentation in volumetric MRI},
  author={Collado, Carlos N{\'a}cher},
  journal={arXiv preprint arXiv:2208.13671},
  year={2022}
}

@article{center2023enmap,
  title={EnMAP Ground Segment},
  author={Center, German Space Operation},
  year={2023}
}

@inproceedings{hu2018squeeze,
  title={Squeeze-and-excitation networks},
  author={Hu, Jie and Shen, Li and Sun, Gang},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={7132--7141},
  year={2018}
}

@inproceedings{woo2018cbam,
  title={Cbam: Convolutional block attention module},
  author={Woo, Sanghyun and Park, Jongchan and Lee, Joon-Young and Kweon, In So},
  booktitle={Proceedings of the European conference on computer vision (ECCV)},
  pages={3--19},
  year={2018}
}

@inproceedings{chollet2017xception,
  title={Xception: Deep learning with depthwise separable convolutions},
  author={Chollet, Fran{\c{c}}ois},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1251--1258},
  year={2017}
}

@article{li2017spectral,
  title={Spectral--spatial classification of hyperspectral imagery with 3D convolutional neural network},
  author={Li, Ying and Zhang, Haokui and Shen, Qiang},
  journal={Remote Sensing},
  volume={9},
  number={1},
  pages={67},
  year={2017},
  publisher={MDPI}
}

@inproceedings{tran2015learning,
  title={Learning spatiotemporal features with 3d convolutional networks},
  author={Tran, Du and Bourdev, Lubomir and Fergus, Rob and Torresani, Lorenzo and Paluri, Manohar},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={4489--4497},
  year={2015}
}

@article{firat2022hybrid,
  title={Hybrid 3D Convolution and 2D Depthwise Separable Convolution Neural Network for Hyperspectral Image Classification},
  author={Firat, H{\"u}seyin and Asker, Mehmet Emin and Hanbay, Davut},
  journal={Balkan Journal of Electrical and Computer Engineering},
  volume={10},
  number={1},
  pages={35--46},
  year={2022},
  publisher={Balkan Yay{\i}n}
}

@mastersthesis{da2022hyperspectral,
  title={Hyperspectral Image Fusion--A Comprehensive Review},
  author={da Lomba Magalh{\~a}es, Miguel Jorge},
  year={2022},
  school={It{\"a}-Suomen yliopisto}
}

@inproceedings{teke2013short,
  title={A short survey of hyperspectral remote sensing applications in agriculture},
  author={Teke, Mustafa and Deveci, H{\"u}sne Seda and Halilo{\u{g}}lu, Onur and G{\"u}rb{\"u}z, Sevgi Z{\"u}beyde and Sakarya, Ufuk},
  booktitle={2013 6th international conference on recent advances in space technologies (RAST)},
  pages={171--176},
  year={2013},
  organization={IEEE}
}

@phdthesis{yohannes2021satellite,
  title={Satellite Based Exploration of Land-Use Dynamics, Drought Susceptibility, and Land Suitability in Central Highlands of Ethiopia},
  author={Yohannes, Moges},
  year={2021},
  school={Addis Ababa University}
}

@article{roy2019hybridsn,
	title={HybridSN: Exploring 3D-2D CNN Feature Hierarchy for Hyperspectral Image Classification},
	author={Roy, Swalpa Kumar and Krishna, Gopal and Dubey, Shiv Ram and Chaudhuri, Bidyut B},
	journal={IEEE Geoscience and Remote Sensing Letters},
	volume={17},
	no.={2},
	pp.={277-281},
	year={2020}
}

@article{melgani2004classification,
  title={Classification of hyperspectral remote sensing images with support vector machines},
  author={Melgani, Farid and Bruzzone, Lorenzo},
  journal={IEEE Transactions on geoscience and remote sensing},
  volume={42},
  number={8},
  pages={1778--1790},
  year={2004},
  publisher={IEEE}
}

@inproceedings{makantasis2015deep,
  title={Deep supervised learning for hyperspectral data classification through convolutional neural networks},
  author={Makantasis, Konstantinos and Karantzalos, Konstantinos and Doulamis, Anastasios and Doulamis, Nikolaos},
  booktitle={2015 IEEE international geoscience and remote sensing symposium (IGARSS)},
  pages={4959--4962},
  year={2015},
  organization={IEEE}
}

@article{hamida20183,
  title={3-D deep learning approach for remote sensing image classification},
  author={Hamida, Amina Ben and Benoit, Alexandre and Lambert, Patrick and Amar, Chokri Ben},
  journal={IEEE Transactions on geoscience and remote sensing},
  volume={56},
  number={8},
  pages={4420--4434},
  year={2018},
  publisher={IEEE}
}

@inproceedings{he2017multi,
  title={Multi-scale 3D deep convolutional neural network for hyperspectral image classification},
  author={He, Mingyi and Li, Bo and Chen, Huahui},
  booktitle={2017 IEEE International Conference on Image Processing (ICIP)},
  pages={3904--3908},
  year={2017},
  organization={IEEE}
}

@article{zhong2017spectral,
  title={Spectral--spatial residual network for hyperspectral image classification: A 3-D deep learning framework},
  author={Zhong, Zilong and Li, Jonathan and Luo, Zhiming and Chapman, Michael},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={56},
  number={2},
  pages={847--858},
  year={2017},
  publisher={IEEE}
}

@inproceedings{heo2021rethinking,
  title={Rethinking spatial dimensions of vision transformers},
  author={Heo, Byeongho and Yun, Sangdoo and Han, Dongyoon and Chun, Sanghyuk and Choe, Junsuk and Oh, Seong Joon},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={11936--11945},
  year={2021}
}

@article{sun2019spectral,
  title={Spectral--spatial attention network for hyperspectral image classification},
  author={Sun, Hao and Zheng, Xiangtao and Lu, Xiaoqiang and Wu, Siyuan},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={58},
  number={5},
  pages={3232--3245},
  year={2019},
  publisher={IEEE}
}

@article{sun2022spectral,
  title={Spectral--spatial feature tokenization transformer for hyperspectral image classification},
  author={Sun, Le and Zhao, Guangrui and Zheng, Yuhui and Wu, Zebin},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={60},
  pages={1--14},
  year={2022},
  publisher={IEEE}
}

@article{yang2022hyperspectral,
  title={Hyperspectral image transformer classification networks},
  author={Yang, Xiaofei and Cao, Weijia and Lu, Yao and Zhou, Yicong},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={60},
  pages={1--15},
  year={2022},
  publisher={IEEE}
}

@inproceedings{zhang2023quantum,
  title={Quantum-Inspired Spectral-Spatial Pyramid Network for Hyperspectral Image Classification},
  author={Zhang, Jie and Zhang, Yongshan and Zhou, Yicong},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={9925--9934},
  year={2023}
}

@article{wang2021simple,
  title={A simple and efficient reconstruction backbone for snapshot compressive imaging},
  author={Wang, Jiamian and Zhang, Yulun and Yuan, Xin and Fu, Yun and Tao, Zhiqiang},
  journal={arXiv preprint arXiv:2108.07739},
  year={2021}
}

@article{hong2021spectralformer,
  title={SpectralFormer: Rethinking hyperspectral image classification with transformers},
  author={Hong, Danfeng and Han, Zhu and Yao, Jing and Gao, Lianru and Zhang, Bing and Plaza, Antonio and Chanussot, Jocelyn},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={60},
  pages={1--15},
  year={2021},
  publisher={IEEE}
}

@article{li2018discriminant,
  title={Discriminant analysis-based dimension reduction for hyperspectral image classification: A survey of the most recent advances and an experimental comparison of different techniques},
  author={Li, Wei and Feng, Fubiao and Li, Hengchao and Du, Qian},
  journal={IEEE Geoscience and Remote Sensing Magazine},
  volume={6},
  number={1},
  pages={15--34},
  year={2018},
  publisher={IEEE}
}

@article{kumar2020feature,
  title={Feature extraction for hyperspectral image classification: A review},
  author={Kumar, Brajesh and Dikshit, Onkar and Gupta, Ashwani and Singh, Manoj Kumar},
  journal={International Journal of Remote Sensing},
  volume={41},
  number={16},
  pages={6248--6287},
  year={2020},
  publisher={Taylor \& Francis}
}

@article{zhang2020review,
  title={Review on graph learning for dimensionality reduction of hyperspectral image},
  author={Zhang, Liangpei and Luo, Fulin},
  journal={Geo-spatial Information Science},
  volume={23},
  number={1},
  pages={98--106},
  year={2020},
  publisher={Taylor \& Francis}
}

@article{yu2017convolutional,
  title={Convolutional neural networks for hyperspectral image classification},
  author={Yu, Shiqi and Jia, Sen and Xu, Chunyan},
  journal={Neurocomputing},
  volume={219},
  pages={88--98},
  year={2017},
  publisher={Elsevier}
}

@article{shi2022hyperspectral,
  title={Hyperspectral image classification based on spectral multiscale convolutional neural network},
  author={Shi, Cuiping and Sun, Jingwei and Wang, Liguo},
  journal={Remote Sensing},
  volume={14},
  number={8},
  pages={1951},
  year={2022},
  publisher={MDPI}
}

@article{bouchoucha2023robustness,
  title={Robustness assessment of hyperspectral image CNNs using metamorphic testing},
  author={Bouchoucha, Rached and Braiek, Houssem Ben and Khomh, Foutse and Bouzidi, Sonia and Zaatour, Rania},
  journal={Information and Software Technology},
  pages={107281},
  year={2023},
  publisher={Elsevier}
}

@article{signoroni2019deep,
  title={Deep learning meets hyperspectral image analysis: A multidisciplinary review},
  author={Signoroni, Alberto and Savardi, Mattia and Baronio, Annalisa and Benini, Sergio},
  journal={Journal of Imaging},
  volume={5},
  number={5},
  pages={52},
  year={2019},
  publisher={MDPI}
}

@book{rangnekar2022learning,
  title={Learning Representations in the Hyperspectral Domain in Aerial Imagery},
  author={Rangnekar, Aneesh Prasad},
  year={2022},
  publisher={Rochester Institute of Technology}
}

@article{hong2021spectralformer,
  title={SpectralFormer: Rethinking hyperspectral image classification with transformers},
  author={Hong, Danfeng and Han, Zhu and Yao, Jing and Gao, Lianru and Zhang, Bing and Plaza, Antonio and Chanussot, Jocelyn},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={60},
  pages={1--15},
  year={2021},
  publisher={IEEE}
}

@inproceedings{beal2022billion,
  title={Billion-scale pretraining with vision transformers for multi-task visual representations},
  author={Beal, Josh and Wu, Hao-Yu and Park, Dong Huk and Zhai, Andrew and Kislyuk, Dmitry},
  booktitle={Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision},
  pages={564--573},
  year={2022}
}

@inproceedings{zhang2021multi,
  title={Multi-scale vision longformer: A new vision transformer for high-resolution image encoding},
  author={Zhang, Pengchuan and Dai, Xiyang and Yang, Jianwei and Xiao, Bin and Yuan, Lu and Zhang, Lei and Gao, Jianfeng},
  booktitle={Proceedings of the IEEE/CVF international conference on computer vision},
  pages={2998--3008},
  year={2021}
}

@article{cai2022semi,
  title={Semi-supervised vision transformers at scale},
  author={Cai, Zhaowei and Ravichandran, Avinash and Favaro, Paolo and Wang, Manchen and Modolo, Davide and Bhotika, Rahul and Tu, Zhuowen and Soatto, Stefano},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={25697--25710},
  year={2022}
}

@article{singh2014quality,
  title={Quality metrics evaluation of hyperspectral images},
  author={Singh, Arvind Kumar and Kumar, HV and Kadambi, Govind R and Kishore, JK and Shuttleworth, James and Manikandan, J},
  journal={The International Archives of the Photogrammetry, Remote Sensing and Spatial Information Sciences},
  volume={40},
  pages={1221--1226},
  year={2014},
  publisher={Copernicus GmbH}
}

@article{deborah2015comprehensive,
  title={A comprehensive evaluation of spectral distance functions and metrics for hyperspectral image processing},
  author={Deborah, Hilda and Richard, No{\"e}l and Hardeberg, Jon Yngve},
  journal={IEEE Journal of Selected Topics in Applied Earth Observations and Remote Sensing},
  volume={8},
  number={6},
  pages={3224--3234},
  year={2015},
  publisher={IEEE}
}

@inproceedings{chaithra2018survey,
  title={A Survey on Image Fusion Techniques and Performance Metrics},
  author={Chaithra, CC and Taranath, NL and Darshan, LM and Subbaraya, CK},
  booktitle={2018 Second International Conference on Electronics, Communication and Aerospace Technology (ICECA)},
  pages={995--999},
  year={2018},
  organization={IEEE}
}

